Chill-Pass: Using Neuro-Physiological Responses to Chill Music to Defeat Coercion Attacks

Current alphanumeric and biometric authentication systems cannot withstand situations where a user is coerced into releasing their authentication materials under hostile circumstances. Existing approaches of coercion resistant authentication systems (CRAS) propose authentication factors such as implicit learning tasks, which are non-transferable, but still have the drawback that an attacker can force the victim (causing stress) to perform the task in order to gain unauthorized access. Alternatively, there could be cases where the user could claim that they were coerced into giving up the authentication materials, whereas in reality they acted as an insider attacker. Therefore, being able to detect stress during authentication also helps to achieve non-repudiation in such cases. To address these concerns, we need CRAS that have both the non-transferable property as well as a mechanism to detect stress related to coercion. In this paper, we study the feasibility of using Chill (intensely pleasurable) music as a stimulus to elicit unique neuro-physiological responses that can be used as an authenticating factor for CRAS. Chill music and stress are both stimuli for a neuro-chemical called Dopamine. However, they release the Dopamine at different parts of the brain, resulting in different neuro-physiological responses, which gives us both the non-transferable and stress-detection properties necessary for CRAS. We have experimentally validated our proposed Chill music based CRAS using human subjects and measuring their neuro-physiological responses on our prototype system. Based on the 100 samples collected from the subjects, we were able to successfully authenticate the subjects with an accuracy of over 90\%. Our work not only demonstrates the potential of Chill music as a unique stimulus for CRAS, but also paves the path of wider adoption of CRAS in general.

==> authentication_phase.tex <==
After registration, a user can later authenticate themselves into the system by producing neuro-physiological responses that match those collected during the registration phase. Optionally, baseline responses can also be taken to verify the user attempting to authenticate is not obviously different from the one registered. When a user wishes to authenticate, music can be selected randomly from the available registered Chill music segments and played to the user while their neuro-physiological responses are monitored. Authentication can then be granted or denied based on whether or not the correlation between the registered and monitored neuro-physiological responses are adequately similar. If multiple pieces of music are available, this process may be repeated multiple times in order to increase the accuracy of authentication. Figure~\ref{fig:taphase} illustrates this process.


==> biometric_authentication.tex <==
Although it is important that a coercion resistant authentication system can differentiate between a coerced and normal (non-coerced) user, it is equally important that it defends against other common attack vectors. This is because if it was possible to compromise the system using a simpler attack vector, the system's coercion resistant quality would not be helpful. To address this, in the following sections we discuss weaknesses with standard biometric authentication systems, and how our state-dependent biometric strategy addresses these weaknesses.

\subsubsection{Weaknesses with Standard Biometrics}
Biometric passwords can be described as authentication methods that use a physical identifiers in order to provide authentication. Common biometric passwords include fingerprint and iris scanning, and are much more difficult to compromise than alphanumeric passwords which rely on users memorizing long and random passwords to provide high levels of security. However, one major shortcoming is that they are often unable to be used in mobile environments and are generally used in secured offices and other sites where authentication is required on-site instead of online. This trend seems to be changing with fingerprint scanners on laptops and phones which will quite possibly allow for widespread online biometric authentication similar to current alphanumeric authentication. A major benefit of using biometric authentication is that they cannot be forgotten because they are inherent to a user. This also sometimes becomes a weakness because if a biometric is compromised, it cannot be changed. \\
\indent In order to use biometrics in our coercion resistant authentication system, it is important that we address this weakness, so that a biometric cannot be trivially compromised. This issue occurs because standard biometrics such as fingerprints can be stolen (especially during coercion) and then used to authenticate in the user's place. The possible transfer of a biometric from a victim to an attacker is unacceptable in the case of coercion resistant authentication, so we address this concern by using a state-dependent biometric strategy that substantially decreases the possibility of a biometric being compromised.

\subsubsection{State-Dependent Biometrics}
State-dependent biometrics refer to biometric signatures that are only present when the user is in a certain state. Unlike a fingerprint, the heart rate of a person varies during various activities. If a person is running at a certain pace, their heart rate differs from their normal pattern, but nevertheless has a pattern of its own. By using this principle, we can protect biometrics from being stolen during activities not necessary for authentication by using a biometric that is only stimulated during the time of authentication. Using the previous example, if the users heart rate while running at a certain pace was necessary for authentication, then it could not be stolen from the user in situations where they are not running at that pace. For use in our coercion resistant authentication system, as long as the state required for authentication cannot be achieved while coerced, then it cannot be stolen from a victim during coercion.

==> coercion_keygen.tex <==
Another method of coercion resistant authentication which has been suggested is the use of skin conductance, as well as other factors, in order to generate a password key \cite{gupta2010fighting}. The idea of the key is that it will be generated by either the user's voice, skin conductance, or a combination of both. When the same key is generated as the stored one then the authentication is a success, but if the user is under the stress of coercion, the key will not generate correctly and the authentication will fail. \\
\indent The use of skin conductance as the physiological response of choice can be supported by our previous explanation of the different uses of our chosen physiological responses. Skin conductance is chosen because it reacts quickly to stress and is not influenced by many other factors. Because the environment is not controlled like ours, it is important that the physiological measurements don't have many inconsistencies which can be caused by normal outside factors. \\
\indent During key generation, collected responses are assigned into ranges and these ranges are used in order to gain a value from the lookup table. Some of the values collected are meant to be junk values in order to prevent false authentication, while others are critical values that would invalidate the key if inconsistent. By using a lookup table with a combination of critical and junk values, a secured key can be generated and reproduced easily. \\
\indent With a combination of voice and skin conductance, false negative rates are small, with higher false positive rates. Although too significant to be used in an authentication system of their own, the results prove the plausibility of a coercion resistant system based on physiological responses. \\
\indent Shortcomings of this work are that both of the selected criteria for authentication can be easily stolen in an acceptable state. Because skin conductance is used without being under stimulus, and it is not feasible to prevent against using machine assisted results during authentication, a user's skin conductance can be monitored during a normal state by an attacker and then used to authenticate themself falsely. This type of social engineering attack would utilize tricking a user into measuring their skin conductance or otherwise monitoring the user's skin conductance when they were unaware of it. Similarly, a user's voice is easy to obtain through social engineering or other simple methods. \\
\indent Our research focuses on enhancing the practicality of a physiological based coercion resistant authentication system. By using stimulated physiological responses, we are able to prevent against the easy theft of critical authentication material. By doing so, we stray away from the use of standard biometrics and incorporate the idea of key dependent biometrics. This idea being that a biometric would only be correct given the correct circumstances, the correct circumstances being during the authentication period. 

==> deap.tex <==
As mentioned before, the DEAP data set is a collection of physiological responses of different users to music videos \cite{koelstra2012deap}. In their research, they use these collected physiological responses, as well as users self reported information, in order to try and classify the user's liking of a music video by their physiological responses. \\
\indent After developing a data set including the reactions of each user to all different music videos, the self reported liking values correlating to each user-video combination were used. Random samples of user-video combinations and their correlating self reported liking were used in order to develop a training set . Various methods were then used in order to attempt to minimize the subjectivity of a user's self reported liking. \\
\indent By using a Spearman correlation coefficient to relate the user-video combinations to their self reported likings, algorithms for correlating physiological responses to expected liking values were developed. Finally, the user-video combinations not used for the training period were input into their system and expected liking values were output. The expected liking values were then compared to the self reported liking values in order to test the accuracy of their classifications. \\
\indent In the best case scenario, about 60\% of the classifications were positive. In a single trial classification system, this is quite impressive, and they were able to prove the feasibility of classifying emotions based on physiological responses. \\
\indent The shortcomings of this work can mostly be attributed to the single trial system. Given multiple trials, more accurate estimations could have been produced. Also, because of the subjectivity of the self reported liking, the accuracy was affected negatively. \\ 
\indent In our work, we use many of the methods demonstrated in the DEAP paper in order to determine the accuracy of our hypotheses. In theory, coercion is simply an emotion experienced by the user, so the ability to classify emotion based on physiological responses was imperative to our work on coercion resistant authentication.

==> experimental_procedure.tex <==
TEST

==> neuro_crypto.tex <==
One of the first attempts at coercion resistant authentication focuses on implicit learning and the ability to be unable to convey a password to another \cite{bojinov2012neuroscience}. This idea is the main focus of coercion resistant authentication because it prevents a user from giving an attacker useful information in order to falsify authentication. This research focuses on the human memory and how to use implicit learning to teach a user to do a specific task in a way they do not explicitly understand. \\
\indent In this research, subjects were given a computerized game similar to the popular "Guitar Hero" game. Essentially, there were many slots that correlated to different keys on a keyboard and dots would fall from the screen into these slots. When a dot aligned with a slot, the subject was supposed to hit the key correlating to the slot in order to gain points for that dot. The order in which the dots fell varied depending on patterns which were determined during the training phase. \\
\indent To prevent false authentication, during authentication a pattern was randomly chosen to be used from a pool of known and unknown patterns for the user. This prevented someone experienced in the game from being able to always win and gain access. Because the authentication was based on the user's motor skills, the original learning of their patterns could be compared to riding a bicycle. They were able to accurately perform when given the pattern, however were not able to explain to others how the pattern worked. \\
\indent Safety precautions were taken in order to avoid an attacker learning a pattern or using the little information that a user could remember from a pattern in order to reconstruct it accurately. They also accounted for an attacker using the system just to see multiple patterns so that they could learn them in the future. \\
\indent In order to check the reliability of the implicit learning strategy over time, they waited for two, one-week long periods. After the first one-week period they had some subjects try to authenticate. After another week they had more users, who had not authenticated for the past two weeks, try to authenticate. The purpose was to determine what the decay of accuracy would be over these lapses in time. They found that after the first week there was noticeable decay in the subject's ability to authenticate themselves, but after the second week the decay was only slightly more significant. Furthermore, they were able to gain better accuracy in authentication if a longer authentication period was administered. \\
\indent Overall the shortcomings of this work are mainly the decay of accuracy over a relatively short period of nonuse. The system also only has the ability to prevent against coercion attacks used to gain information from a user instead of coercion attacks used to force a user to authenticate. \\
\indent As mentioned earlier, our research focuses on more levels of coercion attacks, as we are not only able to deter against coercion that tries to gain information from a user, but also coercion that is used to force a user to authenticate themselves in both the long and short term. \\
\indent We also try to focus more on the repeatability of our system over long periods of time. By using the stimulus of chill music, we attempt to preserve results over longer periods of non use. Although we do plan to cycle through pieces of music every six months, a period of one month of non use shouldn't cause a significant decay in results that would throw off the authentication process.

==> proposed_system.tex <==
Our proposed CRAS is designed provide both an accurate authentication method and resistance against coercion-based attacks. This system is based off of neuro-physiological responses to music, and requires a user to register their neuro-physiological responses into the system before being able to authenticate. The neuro-physiological responses monitored by the system, and how the system conducts it's registration and authentication phases are covered in detail below.

==> security_considerations.tex <==
Because the system is based on physiological and neurological responses being consistent, there has to be consideration for physically altering experiences. Although these situations are limited, mental illness and/or extreme physical trauma can reduce the accuracy of our authentication system. Furthermore, because we add new users to the system, replace hardware components, and change authentication material over time, we need to consider all of the security implications connected with these tasks. In this section we will discuss various security standards associated with the system designed in order to prevent breaches in security.

\subsubsection{Initial Set-Up}
During the installment of the security system, the first step is to select the super users (or system administrators). There must be at least 2 and can be as many as necessary, however, the number of super users can distract from the security as a whole. We use at least 2 super users to make sure that even if a single user is compromised, the system as a whole is unaffected. When selecting super users it is important to choose those who would be extremely difficult to attack or otherwise compromise. The idea should be that if two or more of the super users are successfully compromised, you may have more to worry about than the security system failing.

\subsubsection{Super Users}
Super users have access to add new users, delete users, reset passwords (redo registration), or otherwise add/delete specific pieces of music or privileges from users. However, a super user can only gain access by going through a special two-man authentication process. \\
\indent In order to preserve the integrity of the system as a coercion resistant system, two super users must be present in order to gain administrative access to the system. In order to authenticate themselves, they must simultaneously present fingerprint and iris scans as well as human verification. The human verification method will be elaborated on in future research but will focus on physiological and neurological responses in order to determine that a machine is not attempting to spoof a biometric authentication method. These functionalities will be built in, instead of attachable and destructible like the physiological and neurological monitors. This will prevent the system from having no method of authentication if the attachable authentication hardware malfunction.

\subsubsection{Repalcements}
In order to maintain integrity, some hardware components are destructible to prevent tampering. Because headphones and physiological and neurological monitors are attached to a user, they need to be impossible to tamper, and therefore break whenever an attempt is made to view the interior of the device. This is unlike the physiological and neurological monitors used for the super users which are built into the system and do not have to attach to a user. \\
\indent In order to replace any hardware, users or music in the system, super user administration is necessary. After super user access is granted, any kind of replacement becomes possible. When replacing equipment it is optimal that the party responsible for breaking it isn't involved, this is not mandatory however is highly suggested.
